Yield and Buckling Stress Limits in Topology Optimization of Multiscale Structures

This study presents an extension of multiscale topology optimization by integrating both yield stress and local/global buckling considerations into the design process. Building upon established multiscale methodologies, we develop a new framework incorporating yield stress limits either as constraints or objectives alongside previously established local and global buckling constraints. This approach significantly refines the optimization process, ensuring that the resulting designs meet mechanical performance criteria and adhere to critical material yield constraints. First, we establish local density-dependent von Mises yield surfaces based on local yield estimates from homogenization-based analysis to predict the local yield limits of the homogenized materials. Then, these local Yield-based Load Factors (YLFs) are combined with local and global buckling criteria to obtain topology optimized designs that consider yield and buckling failure on all levels. This integration is crucial for the practical application of optimized structures in real-world scenarios, where material yield and stability behavior critically influence structural integrity and durability. Numerical examples demonstrate how optimized designs depend on the stiffness to yield ratio of the considered building material. Despite the foundational assumption of separation of scales, the de-homogenized structures, even at relatively coarse length scales, exhibit a high degree of agreement with the corresponding homogenized predictions.

==> figures/YieldParmaterAnalysis/maxParameters.tex <==
\begin{tikzpicture}
    \begin{axis}[
        xlabel = {$\bar{\eta}$},
        ylabel = {$\alpha$},
        legend pos = south west,
        xmin=0, xmax=1.25,
        ymin=-0.65, ymax=0.22,
        width=6cm,   % Set the width of the plot
        height=5.45cm,    % Set the height of the plot
        xmajorgrids=true,
        ymajorgrids=true,
        % legend style={at={(1.05,0.5)}, anchor=west}, % Place legend outside
        % yticklabel style={
        %     /pgf/number format/fixed,
        %     /pgf/number format/precision=2,
        %     % rotate=90 % Rotate the y-axis tick labels
        % },
        % scaled y ticks=false, % Disable scientific notation on x-axis
        % xticklabel style={
        %     /pgf/number format/fixed,
        %     /pgf/number format/precision=2,
        %     % rotate=90 % Rotate the y-axis tick labels
        % },
        % scaled x ticks=false, % Disable scientific notation on x-axis0
    ]
    

    \addplot+[
    color=mycolor3,
    only marks,
    mark=*,
    fill=mycolor3,
    mark options={solid},
    mark size = 1pt, % Adjust the size of the markers
    legend image post style={mark size=2pt} % Adjust the size of the markers in the legend
    ]
    table [x index=0, y index=1, col sep=comma] {figures/YieldParmaterAnalysis/maxE_Coord.csv};
    \addlegendentry{$max(\bar{E})$}

    \addplot+[
    color=mycolor1,
    only marks,
    mark=*,
    fill=mycolor1,
    mark options={solid},
    mark size = 1pt, % Adjust the size of the markers
    legend image post style={mark size=2pt} % Adjust the size of the markers in the legend
    ]
    table [x index=0, y index=1, col sep=comma] {figures/YieldParmaterAnalysis/maxVM_Coord.csv};
    \addlegendentry{$max(\sigma_y)$}

    
    % \node at (axis cs:2.0000, 0.0206) [circle,fill=mycolor1,inner sep=1.5pt]{};
    % \node at (axis cs:2.0000, 0.0206) [anchor=north, color=black] {$\lambda_{crit}$};
    \end{axis}
\end{tikzpicture}%
